A Spitzer Survey for Dust-Obscured Supernovae

Supernova (SN) rates serve as an important probe of star-formation models and initial mass functions. Near-infrared seeing-limited ground-based surveys typically discover a factor of 3-10 fewer SNe than predicted from far-infrared (FIR) luminosities owing to sensitivity limitations arising from both a variable point-spread function (PSF) and high dust extinction in the nuclear regions of star-forming galaxies. This inconsistency has potential implications for our understanding of star-formation rates and massive-star evolution, particularly at higher redshifts, where star-forming galaxies are more common. To resolve this inconsistency, a successful SN survey in the local universe must be conducted at longer wavelengths and with a space-based telescope, which has a stable PSF to reduce the necessity for any subtraction algorithms and thus residuals. Here we report on a two-year Spitzer/IRAC 3.6 um survey for dust-extinguished SNe in the nuclear regions of forty luminous infrared galaxies (LIRGs) within 200 Mpc. The asymmetric Spitzer PSF results in worse than expected subtraction residuals when implementing standard template subtraction. Forward-modeling techniques improve our sensitivity by ~1.5 magnitudes. We report the detection of 9 SNe, five of which were not discovered by optical surveys. After adjusting our predicted rates to account for the sensitivity of our survey, we find that the number of detections is consistent with the models. While this search is nonetheless hampered by a difficult-to-model PSF and the relatively poor resolution of Spitzer, it will benefit from future missions, such as Roman Space Telescope and JWST, with higher resolution and more symmetric PSFs.

==> tab_spitz.tex <==
\begin{tabular}{lrrrr}
%\toprule
Galaxy &  1\arcsec &  3\arcsec &  5\arcsec &  10\arcsec \\
%\midrule
\hline
NGC 034      &    9.71 &     10.37 &    10.49 &   10.70 \\
NGC 232      &    9.30 &      9.92 &    10.22 &   10.58 \\
MCG+12-02   &    9.22 &     10.04 &    10.33 &   10.66 \\
IC 1623      &    8.92 &      9.78 &    10.09 &   10.59 \\
UGC 2369     &    8.95 &      9.60 &     9.97 &   10.57 \\
IRAS 03359   &    9.69 &     10.34 &    10.50 &   10.84 \\
MCG-03-12   &    9.36 &     10.05 &    10.27 &   10.62 \\
NGC 1572     &    9.39 &     10.06 &    10.18 &   10.46 \\
NGC 1614     &    9.54 &     10.39 &    10.58 &   10.81 \\
NGC 2623     &    9.56 &     10.16 &    10.33 &   10.63 \\
UGC 4881     &    9.68 &     10.33 &    10.53 &   10.91 \\
UGC 5101     &   10.20 &     10.78 &    10.89 &   11.14 \\
MCG+08-18   &    8.24 &      9.06 &     9.34 &    9.85 \\
IC 563       &    8.78 &      9.56 &     9.82 &   10.26 \\
NGC 3110     &    9.11 &      9.87 &    10.06 &   10.40 \\
NGC 3256     &    9.32 &     10.08 &    10.35 &   10.72 \\
IRAS 10565   &   10.22 &     10.85 &    10.95 &   11.22 \\
Arp 148      &    9.69 &     10.33 &    10.49 &   10.80 \\
MCG+00-29   &    9.62 &     10.27 &    10.39 &   10.65 \\
IC 2810      &    9.63 &     10.25 &    10.42 &   10.77 \\
NGC 3690     &    9.30 &     10.11 &    10.35 &   10.70 \\
ESO 507-G070 &    9.43 &     10.11 &    10.28 &   10.61 \\
UGC 8335     &    8.89 &      9.55 &     9.71 &    9.82 \\
UGC 8387     &    9.67 &     10.38 &    10.55 &   10.83 \\
NGC 5256     &    9.04 &      9.81 &    10.25 &   10.70 \\
NGC 5257     &    8.98 &      9.65 &     9.92 &   10.42 \\
Mk 273       &   10.36 &     10.95 &    11.11 &   11.41 \\
NGC 5331     &    9.62 &     10.34 &    10.51 &   10.84 \\
UGC 8782     &    9.31 &      9.94 &    10.07 &   10.39 \\
Arp 302      &    9.67 &     10.37 &    10.57 &   10.89 \\
Mk 848       &   10.05 &     10.68 &    10.80 &   11.07 \\
Arp 220      &    9.75 &     10.41 &    10.49 &   10.57 \\
NGC 6090     &    9.09 &      9.88 &    10.20 &   10.72 \\
NGC 6240     &   10.04 &     10.67 &    10.78 &   11.00 \\
IRAS 17208   &   10.38 &     11.02 &    11.16 &   11.47 \\
IC 4687      &    9.34 &     10.14 &    10.35 &   10.61 \\
IRAS 18293   &    9.74 &     10.48 &    10.68 &   10.98 \\
NGC 6926     &    8.80 &      9.47 &     9.72 &   10.21 \\
NGC 7130     &    9.41 &     10.06 &    10.22 &   10.53 \\
IRAS 23128   &   10.13 &     10.77 &    10.92 &   11.19 \\
%\bottomrule
\end{tabular}

